K2-19b and c are in a 3:2 Commensurability but out of Resonance: A Challenge to Planet Assembly by Convergent Migration

K2-19b and c were among the first planets discovered by NASA's K2 mission and together stand in stark contrast with the physical and orbital properties of the solar system planets. The planets are between the size of Uranus and Saturn at 7.0$\pm$0.2 R_E and 4.1$\pm$0.2 R_E, respectively, and reside a mere 0.1% outside the nominal 3:2 mean-motion resonance. They represent a different outcome of the planet formation process than the solar system, as well as the vast majority of known exoplanets. We measured the physical and orbital properties of these planets using photometry from K2, Spitzer, and ground-based telescopes, along with radial velocities from Keck/HIRES. Through a joint photodynamical model, we found that the planets have moderate eccentricities of $e \approx0.20$ and well-aligned apsides $\Delta \varpi \approx 0$ deg. The planets occupy a strictly non-resonant configuration: the resonant angles circulate rather than librate. This defies the predictions of standard formation pathways that invoke convergent or divergent migration, both of which predict $\Delta \varpi \approx 180$ deg and eccentricities of a few percent or less. We measured masses of $M_{p,b}$ = 32.4$\pm$1.7 M_E and $M_{p,c}$ = 10.8$\pm$0.6 M_E. Our measurements, with 5% fractional uncertainties, are among the most precise of any sub-Jovian exoplanet. Mass and size reflect a planet's core/envelope structure. Despite having a relatively massive core of $M_{core} \approx15$ $M_E$, K2-19b is envelope-rich, with an envelope mass fraction of roughly 50%. This planet poses a challenge to standard models core-nucleated accretion, which predict that cores $\gtrsim 10$ $M_E$ will quickly accrete gas and trigger runaway accretion when the envelope mass exceeds that of the core.

==> tab_rv.tex <==
2225.996346 & -8.92 & 2.69 & 0.358 \\
2229.058283 & -14.53 & 2.84 & 0.328 \\
2346.849965 & -11.35 & 1.98 & 0.181 \\
2366.792920 & -0.21 & 2.04 & 0.247 \\
2367.829151 & -9.39 & 3.37 & 0.221 \\
2368.814357 & -14.07 & 2.20 & 0.182 \\
2370.809676 & -18.62 & 2.13 & 0.221 \\
2374.805352 & 6.22 & 3.15 & 0.195 \\
2375.803685 & 2.94 & 2.18 & 0.249 \\
2376.797458 & -14.34 & 2.12 & 0.269 \\
2377.781696 & -27.89 & 2.18 & 0.234 \\
2380.787799 & 5.63 & 2.59 & 0.229 \\
2382.794564 & 10.68 & 2.74 & 0.265 \\
2383.795563 & 2.58 & 2.86 & 0.261 \\
2384.777433 & -17.71 & 2.34 & 0.263 \\
2396.763375 & -16.29 & 3.79 & 0.214 \\
2397.761910 & 3.55 & 3.40 & 0.245 \\
2521.131634 & -20.61 & 2.68 & 0.253 \\
2547.147573 & 13.11 & 2.22 & 0.261 \\
2569.119539 & -5.66 & 2.12 & 0.272 \\
2579.059045 & -11.43 & 2.14 & 0.260 \\
2580.019920 & -4.31 & 2.54 & 0.234 \\
2590.075158 & 1.22 & 2.07 & 0.286 \\
2913.066679 & 11.78 & 2.56 & 0.278 \\
2914.053271 & 7.69 & 1.97 & 0.289 \\
2915.070270 & -3.48 & 2.42 & 0.293 \\
2927.038832 & -11.88 & 2.47 & 0.270 \\
2931.033590 & -6.04 & 1.97 & 0.292 \\
2933.001662 & -9.65 & 2.41 & 0.292 \\
2941.987793 & -10.29 & 1.99 & 0.300 \\
2955.004165 & -5.03 & 2.13 & 0.305 \\
2955.985247 & -8.43 & 2.00 & 0.307 \\
2956.988020 & -12.47 & 1.91 & 0.309 \\
2957.921886 & 0.04 & 2.04 & 0.401 \\
2959.993470 & 12.32 & 2.41 & 0.294 \\
2961.003460 & -1.85 & 2.03 & 0.308 \\
2961.946419 & -3.57 & 2.10 & 0.311 \\
2969.899343 & 2.35 & 1.96 & 0.303 \\
2970.880172 & 0.31 & 2.33 & 0.282 \\
2972.897779 & 4.33 & 2.33 & 0.307 \\
2973.897551 & 0.58 & 2.16 & 0.294 \\
2995.864123 & -17.42 & 2.15 & 0.288 \\
2996.957641 & -13.52 & 1.89 & 0.291 \\
2997.877871 & 0.21 & 2.08 & 0.301 \\
3021.905244 & -2.47 & 2.31 & 0.287 \\
3053.848016 & 5.39 & 1.97 & 0.274 \\
3092.825866 & -10.14 & 2.28 & 0.285 \\
3093.840536 & 8.50 & 1.93 & 0.276 \\
3259.112368 & 15.11 & 2.09 & 0.333 \\
3280.131860 & 14.55 & 1.98 & 0.338 \\
3281.110002 & 12.98 & 2.03 & 0.334 \\

==> tab_transit-times-predict.tex <==
b & 0 & 2014-06-04 & 1980.3840 & 0.0002 \\
c & 0 & 2014-06-08 & 1984.2722 & 0.0008 \\
b & 1 & 2014-06-12 & 1988.3041 & 0.0002 \\
c & 1 & 2014-06-20 & 1996.1834 & 0.0006 \\
b & 2 & 2014-06-20 & 1996.2220 & 0.0002 \\
b & 3 & 2014-06-28 & 2004.1406 & 0.0002 \\
c & 2 & 2014-07-02 & 2008.0922 & 0.0005 \\
b & 4 & 2014-07-06 & 2012.0614 & 0.0001 \\
b & 5 & 2014-07-14 & 2019.9801 & 0.0001 \\
c & 3 & 2014-07-14 & 2020.0007 & 0.0004 \\
b & 6 & 2014-07-22 & 2027.8992 & 0.0002 \\
c & 4 & 2014-07-26 & 2031.9067 & 0.0004 \\
b & 7 & 2014-07-30 & 2035.8204 & 0.0002 \\
b & 8 & 2014-08-07 & 2043.7393 & 0.0002 \\
c & 5 & 2014-08-07 & 2043.8125 & 0.0005 \\
b & 9 & 2014-08-15 & 2051.6586 & 0.0002 \\
c & 6 & 2014-08-19 & 2055.7158 & 0.0006 \\
b & 10 & 2014-08-23 & 2059.5803 & 0.0002 \\
b & 11 & 2014-08-31 & 2067.5001 & 0.0002 \\
c & 7 & 2014-08-31 & 2067.6189 & 0.0009 \\
b & 12 & 2014-09-07 & 2075.4200 & 0.0003 \\
c & 8 & 2014-09-12 & 2079.5196 & 0.0010 \\
b & 13 & 2014-09-15 & 2083.3421 & 0.0003 \\
b & 14 & 2014-09-23 & 2091.2620 & 0.0003 \\
c & 9 & 2014-09-23 & 2091.4202 & 0.0013 \\
b & 15 & 2014-10-01 & 2099.1820 & 0.0004 \\
c & 10 & 2014-10-05 & 2103.3186 & 0.0015 \\
b & 16 & 2014-10-09 & 2107.1045 & 0.0004 \\
b & 17 & 2014-10-17 & 2115.0251 & 0.0005 \\
c & 11 & 2014-10-17 & 2115.2169 & 0.0018 \\
b & 18 & 2014-10-25 & 2122.9457 & 0.0005 \\
c & 12 & 2014-10-29 & 2127.1132 & 0.0019 \\
b & 19 & 2014-11-02 & 2130.8686 & 0.0005 \\
b & 20 & 2014-11-10 & 2138.7893 & 0.0005 \\
c & 13 & 2014-11-10 & 2139.0095 & 0.0023 \\
b & 21 & 2014-11-18 & 2146.7099 & 0.0006 \\
c & 14 & 2014-11-22 & 2150.9042 & 0.0024 \\
b & 22 & 2014-11-26 & 2154.6329 & 0.0006 \\
b & 23 & 2014-12-04 & 2162.5541 & 0.0006 \\
c & 15 & 2014-12-04 & 2162.7989 & 0.0028 \\
b & 24 & 2014-12-11 & 2170.4752 & 0.0007 \\
c & 16 & 2014-12-16 & 2174.6923 & 0.0029 \\
b & 25 & 2014-12-19 & 2178.3985 & 0.0007 \\
b & 26 & 2014-12-27 & 2186.3199 & 0.0007 \\
c & 17 & 2014-12-28 & 2186.5857 & 0.0032 \\
b & 27 & 2015-01-04 & 2194.2408 & 0.0007 \\
c & 18 & 2015-01-08 & 2198.4784 & 0.0033 \\
b & 28 & 2015-01-12 & 2202.1640 & 0.0007 \\
b & 29 & 2015-01-20 & 2210.0857 & 0.0008 \\
c & 19 & 2015-01-20 & 2210.3710 & 0.0037 \\
b & 30 & 2015-01-28 & 2218.0069 & 0.0008 \\
c & 20 & 2015-02-01 & 2222.2633 & 0.0038 \\
b & 31 & 2015-02-05 & 2225.9304 & 0.0008 \\
b & 32 & 2015-02-13 & 2233.8520 & 0.0008 \\
c & 21 & 2015-02-13 & 2234.1556 & 0.0042 \\
b & 33 & 2015-02-21 & 2241.7729 & 0.0008 \\
c & 22 & 2015-02-25 & 2246.0481 & 0.0043 \\
b & 34 & 2015-03-01 & 2249.6962 & 0.0009 \\
b & 35 & 2015-03-09 & 2257.6178 & 0.0009 \\
c & 23 & 2015-03-09 & 2257.9405 & 0.0047 \\
b & 36 & 2015-03-17 & 2265.5390 & 0.0009 \\
c & 24 & 2015-03-21 & 2269.8336 & 0.0050 \\
b & 37 & 2015-03-24 & 2273.4623 & 0.0010 \\
b & 38 & 2015-04-01 & 2281.3839 & 0.0011 \\
c & 25 & 2015-04-02 & 2281.7266 & 0.0054 \\
b & 39 & 2015-04-09 & 2289.3046 & 0.0011 \\
c & 26 & 2015-04-14 & 2293.6207 & 0.0057 \\
b & 40 & 2015-04-17 & 2297.2274 & 0.0011 \\
b & 41 & 2015-04-25 & 2305.1488 & 0.0012 \\
c & 27 & 2015-04-26 & 2305.5147 & 0.0063 \\
b & 42 & 2015-05-03 & 2313.0695 & 0.0013 \\
c & 28 & 2015-05-07 & 2317.4103 & 0.0067 \\
b & 43 & 2015-05-11 & 2320.9924 & 0.0014 \\
b & 44 & 2015-05-19 & 2328.9136 & 0.0015 \\
c & 29 & 2015-05-19 & 2329.3058 & 0.0073 \\
b & 45 & 2015-05-27 & 2336.8338 & 0.0016 \\
c & 30 & 2015-05-31 & 2341.2032 & 0.0079 \\
b & 46 & 2015-06-04 & 2344.7560 & 0.0017 \\
b & 47 & 2015-06-12 & 2352.6768 & 0.0018 \\
c & 31 & 2015-06-12 & 2353.1004 & 0.0086 \\
b & 48 & 2015-06-20 & 2360.5968 & 0.0019 \\
c & 32 & 2015-06-24 & 2364.9999 & 0.0093 \\
b & 49 & 2015-06-28 & 2368.5190 & 0.0021 \\
b & 50 & 2015-07-05 & 2376.4396 & 0.0022 \\
c & 33 & 2015-07-06 & 2376.8993 & 0.0101 \\
b & 51 & 2015-07-13 & 2384.3591 & 0.0024 \\
c & 34 & 2015-07-18 & 2388.8012 & 0.0109 \\
b & 52 & 2015-07-21 & 2392.2805 & 0.0026 \\
b & 53 & 2015-07-29 & 2400.2005 & 0.0027 \\
c & 35 & 2015-07-30 & 2400.7028 & 0.0117 \\
b & 54 & 2015-08-06 & 2408.1197 & 0.0028 \\
c & 36 & 2015-08-11 & 2412.6073 & 0.0127 \\
b & 55 & 2015-08-14 & 2416.0410 & 0.0031 \\
b & 56 & 2015-08-22 & 2423.9608 & 0.0032 \\
c & 37 & 2015-08-23 & 2424.5113 & 0.0136 \\
b & 57 & 2015-08-30 & 2431.8795 & 0.0034 \\
c & 38 & 2015-09-03 & 2436.4184 & 0.0147 \\
b & 58 & 2015-09-07 & 2439.8000 & 0.0037 \\
b & 59 & 2015-09-15 & 2447.7192 & 0.0038 \\
c & 39 & 2015-09-15 & 2448.3249 & 0.0157 \\
b & 60 & 2015-09-23 & 2455.6374 & 0.0040 \\
c & 40 & 2015-09-27 & 2460.2345 & 0.0169 \\
b & 61 & 2015-10-01 & 2463.5577 & 0.0043 \\
b & 62 & 2015-10-08 & 2471.4768 & 0.0045 \\
c & 41 & 2015-10-09 & 2472.1434 & 0.0180 \\
b & 63 & 2015-10-16 & 2479.3947 & 0.0047 \\
c & 42 & 2015-10-21 & 2484.0555 & 0.0193 \\
b & 64 & 2015-10-24 & 2487.3144 & 0.0051 \\
b & 65 & 2015-11-01 & 2495.2328 & 0.0052 \\
c & 43 & 2015-11-02 & 2495.9665 & 0.0205 \\
b & 66 & 2015-11-09 & 2503.1501 & 0.0054 \\
c & 44 & 2015-11-14 & 2507.8808 & 0.0218 \\
b & 67 & 2015-11-17 & 2511.0696 & 0.0058 \\
b & 68 & 2015-11-25 & 2518.9881 & 0.0059 \\
c & 45 & 2015-11-26 & 2519.7937 & 0.0231 \\
b & 69 & 2015-12-03 & 2526.9053 & 0.0062 \\
c & 46 & 2015-12-08 & 2531.7099 & 0.0245 \\
b & 70 & 2015-12-11 & 2534.8243 & 0.0066 \\
b & 71 & 2015-12-19 & 2542.7422 & 0.0067 \\
c & 47 & 2015-12-20 & 2543.6242 & 0.0258 \\
b & 72 & 2015-12-27 & 2550.6589 & 0.0069 \\
c & 48 & 2016-01-01 & 2555.5419 & 0.0273 \\
b & 73 & 2016-01-04 & 2558.5777 & 0.0073 \\
b & 74 & 2016-01-11 & 2566.4960 & 0.0075 \\
c & 49 & 2016-01-12 & 2567.4571 & 0.0285 \\
b & 75 & 2016-01-19 & 2574.4127 & 0.0077 \\
c & 50 & 2016-01-24 & 2579.3756 & 0.0301 \\
b & 76 & 2016-01-27 & 2582.3312 & 0.0081 \\
b & 77 & 2016-02-04 & 2590.2493 & 0.0082 \\
c & 51 & 2016-02-05 & 2591.2910 & 0.0313 \\
b & 78 & 2016-02-12 & 2598.1656 & 0.0084 \\
c & 52 & 2016-02-17 & 2603.2099 & 0.0328 \\
b & 79 & 2016-02-20 & 2606.0840 & 0.0088 \\
b & 80 & 2016-02-28 & 2614.0025 & 0.0089 \\
c & 53 & 2016-02-29 & 2615.1248 & 0.0339 \\
b & 81 & 2016-03-07 & 2621.9193 & 0.0091 \\
c & 54 & 2016-03-12 & 2627.0433 & 0.0353 \\
b & 82 & 2016-03-15 & 2629.8377 & 0.0094 \\
b & 83 & 2016-03-23 & 2637.7563 & 0.0096 \\
c & 55 & 2016-03-24 & 2638.9570 & 0.0363 \\
b & 84 & 2016-03-31 & 2645.6729 & 0.0097 \\
c & 56 & 2016-04-05 & 2650.8744 & 0.0376 \\
b & 85 & 2016-04-08 & 2653.5913 & 0.0100 \\
b & 86 & 2016-04-16 & 2661.5106 & 0.0100 \\
c & 57 & 2016-04-17 & 2662.7860 & 0.0383 \\
b & 87 & 2016-04-23 & 2669.4278 & 0.0101 \\
c & 58 & 2016-04-29 & 2674.7016 & 0.0394 \\
b & 88 & 2016-05-01 & 2677.3466 & 0.0104 \\
b & 89 & 2016-05-09 & 2685.2664 & 0.0104 \\
c & 59 & 2016-05-11 & 2686.6104 & 0.0397 \\
b & 90 & 2016-05-17 & 2693.1837 & 0.0105 \\
c & 60 & 2016-05-23 & 2698.5235 & 0.0406 \\
b & 91 & 2016-05-25 & 2701.1026 & 0.0107 \\
b & 92 & 2016-06-02 & 2709.0231 & 0.0106 \\
c & 61 & 2016-06-03 & 2710.4289 & 0.0406 \\
b & 93 & 2016-06-10 & 2716.9414 & 0.0106 \\
c & 62 & 2016-06-15 & 2722.3388 & 0.0412 \\
b & 94 & 2016-06-18 & 2724.8609 & 0.0107 \\
b & 95 & 2016-06-26 & 2732.7822 & 0.0106 \\
c & 63 & 2016-06-27 & 2734.2402 & 0.0408 \\
b & 96 & 2016-07-04 & 2740.7008 & 0.0106 \\
c & 64 & 2016-07-09 & 2746.1465 & 0.0410 \\
b & 97 & 2016-07-12 & 2748.6206 & 0.0107 \\
b & 98 & 2016-07-20 & 2756.5425 & 0.0104 \\
c & 65 & 2016-07-21 & 2758.0437 & 0.0401 \\
b & 99 & 2016-07-27 & 2764.4622 & 0.0103 \\
c & 66 & 2016-08-02 & 2769.9460 & 0.0400 \\
b & 100 & 2016-08-04 & 2772.3829 & 0.0103 \\
b & 101 & 2016-08-12 & 2780.3058 & 0.0100 \\
c & 67 & 2016-08-14 & 2781.8386 & 0.0387 \\
b & 102 & 2016-08-20 & 2788.2259 & 0.0099 \\
c & 68 & 2016-08-26 & 2793.7369 & 0.0381 \\
b & 103 & 2016-08-28 & 2796.1469 & 0.0099 \\
b & 104 & 2016-09-05 & 2804.0704 & 0.0095 \\
c & 69 & 2016-09-07 & 2805.6251 & 0.0364 \\
b & 105 & 2016-09-13 & 2811.9914 & 0.0092 \\
c & 70 & 2016-09-19 & 2817.5194 & 0.0355 \\
b & 106 & 2016-09-21 & 2819.9134 & 0.0091 \\
b & 107 & 2016-09-29 & 2827.8378 & 0.0087 \\
c & 71 & 2016-09-30 & 2829.4033 & 0.0335 \\
b & 108 & 2016-10-07 & 2835.7594 & 0.0084 \\
c & 72 & 2016-10-12 & 2841.2939 & 0.0323 \\
b & 109 & 2016-10-15 & 2843.6817 & 0.0083 \\
b & 110 & 2016-10-23 & 2851.6065 & 0.0079 \\
c & 73 & 2016-10-24 & 2853.1741 & 0.0299 \\
b & 111 & 2016-10-31 & 2859.5287 & 0.0075 \\
c & 74 & 2016-11-05 & 2865.0613 & 0.0284 \\
b & 112 & 2016-11-07 & 2867.4519 & 0.0073 \\
b & 113 & 2016-11-15 & 2875.3775 & 0.0068 \\
c & 75 & 2016-11-17 & 2876.9383 & 0.0258 \\
b & 114 & 2016-11-23 & 2883.3001 & 0.0065 \\
c & 76 & 2016-11-29 & 2888.8229 & 0.0241 \\
b & 115 & 2016-12-01 & 2891.2235 & 0.0063 \\
b & 116 & 2016-12-09 & 2899.1492 & 0.0059 \\
c & 77 & 2016-12-11 & 2900.6974 & 0.0214 \\
b & 117 & 2016-12-17 & 2907.0721 & 0.0054 \\
c & 78 & 2016-12-23 & 2912.5800 & 0.0196 \\
b & 118 & 2016-12-25 & 2914.9962 & 0.0052 \\
b & 119 & 2017-01-02 & 2922.9224 & 0.0047 \\
c & 79 & 2017-01-03 & 2924.4528 & 0.0168 \\
b & 120 & 2017-01-10 & 2930.8457 & 0.0043 \\
c & 80 & 2017-01-15 & 2936.3342 & 0.0150 \\
b & 121 & 2017-01-18 & 2938.7697 & 0.0041 \\
b & 122 & 2017-01-26 & 2946.6957 & 0.0037 \\
c & 81 & 2017-01-27 & 2948.2062 & 0.0122 \\
b & 123 & 2017-02-03 & 2954.6188 & 0.0033 \\
c & 82 & 2017-02-08 & 2960.0873 & 0.0105 \\
b & 124 & 2017-02-11 & 2962.5432 & 0.0030 \\
b & 125 & 2017-02-18 & 2970.4695 & 0.0026 \\
c & 83 & 2017-02-20 & 2971.9593 & 0.0079 \\
b & 126 & 2017-02-26 & 2978.3927 & 0.0023 \\
c & 84 & 2017-03-04 & 2983.8409 & 0.0063 \\
b & 127 & 2017-03-06 & 2986.3168 & 0.0021 \\
b & 128 & 2017-03-14 & 2994.2427 & 0.0018 \\
c & 85 & 2017-03-16 & 2995.7138 & 0.0040 \\
b & 129 & 2017-03-22 & 3002.1654 & 0.0015 \\
c & 86 & 2017-03-28 & 3007.5967 & 0.0029 \\
b & 130 & 2017-03-30 & 3010.0894 & 0.0013 \\
b & 131 & 2017-04-07 & 3018.0154 & 0.0010 \\
c & 87 & 2017-04-08 & 3019.4713 & 0.0020 \\
b & 132 & 2017-04-15 & 3025.9380 & 0.0008 \\
c & 88 & 2017-04-20 & 3031.3564 & 0.0023 \\
b & 133 & 2017-04-23 & 3033.8616 & 0.0007 \\
b & 134 & 2017-05-01 & 3041.7868 & 0.0007 \\
c & 89 & 2017-05-02 & 3043.2333 & 0.0037 \\
b & 135 & 2017-05-09 & 3049.7086 & 0.0007 \\
c & 90 & 2017-05-14 & 3055.1212 & 0.0043 \\
b & 136 & 2017-05-17 & 3057.6317 & 0.0007 \\
b & 137 & 2017-05-25 & 3065.5568 & 0.0008 \\
c & 91 & 2017-05-26 & 3067.0011 & 0.0056 \\
b & 138 & 2017-06-01 & 3073.4783 & 0.0008 \\
c & 92 & 2017-06-07 & 3078.8924 & 0.0058 \\
b & 139 & 2017-06-09 & 3081.4009 & 0.0009 \\
b & 140 & 2017-06-17 & 3089.3252 & 0.0010 \\
c & 93 & 2017-06-19 & 3090.7757 & 0.0068 \\
b & 141 & 2017-06-25 & 3097.2457 & 0.0010 \\
c & 94 & 2017-07-01 & 3102.6708 & 0.0066 \\
b & 142 & 2017-07-03 & 3105.1675 & 0.0010 \\
b & 143 & 2017-07-11 & 3113.0914 & 0.0010 \\
c & 95 & 2017-07-13 & 3114.5579 & 0.0071 \\
b & 144 & 2017-07-19 & 3121.0116 & 0.0010 \\
c & 96 & 2017-07-24 & 3126.4571 & 0.0064 \\
b & 145 & 2017-07-27 & 3128.9329 & 0.0010 \\
b & 146 & 2017-08-04 & 3136.8560 & 0.0010 \\
c & 97 & 2017-08-05 & 3138.3481 & 0.0064 \\
b & 147 & 2017-08-12 & 3144.7751 & 0.0009 \\
c & 98 & 2017-08-17 & 3150.2514 & 0.0053 \\
b & 148 & 2017-08-20 & 3152.6954 & 0.0009 \\
b & 149 & 2017-08-28 & 3160.6181 & 0.0009 \\
c & 99 & 2017-08-29 & 3162.1463 & 0.0049 \\
b & 150 & 2017-09-05 & 3168.5370 & 0.0008 \\
c & 100 & 2017-09-10 & 3174.0536 & 0.0035 \\
b & 151 & 2017-09-12 & 3176.4567 & 0.0009 \\
b & 152 & 2017-09-20 & 3184.3788 & 0.0010 \\
c & 101 & 2017-09-22 & 3185.9521 & 0.0029 \\
b & 153 & 2017-09-28 & 3192.2967 & 0.0012 \\
c & 102 & 2017-10-04 & 3197.8631 & 0.0023 \\
b & 154 & 2017-10-06 & 3200.2155 & 0.0014 \\
b & 155 & 2017-10-14 & 3208.1371 & 0.0015 \\
c & 103 & 2017-10-16 & 3209.7650 & 0.0030 \\
b & 156 & 2017-10-22 & 3216.0549 & 0.0018 \\
c & 104 & 2017-10-28 & 3221.6793 & 0.0048 \\
b & 157 & 2017-10-30 & 3223.9733 & 0.0021 \\
b & 158 & 2017-11-07 & 3231.8944 & 0.0024 \\
c & 105 & 2017-11-09 & 3233.5840 & 0.0066 \\
b & 159 & 2017-11-15 & 3239.8116 & 0.0028 \\
c & 106 & 2017-11-21 & 3245.5010 & 0.0093 \\
b & 160 & 2017-11-23 & 3247.7291 & 0.0033 \\
b & 161 & 2017-12-01 & 3255.6498 & 0.0036 \\
c & 107 & 2017-12-02 & 3257.4081 & 0.0117 \\
b & 162 & 2017-12-09 & 3263.5669 & 0.0040 \\
c & 108 & 2017-12-14 & 3269.3271 & 0.0148 \\
b & 163 & 2017-12-16 & 3271.4844 & 0.0045 \\
b & 164 & 2017-12-24 & 3279.4050 & 0.0050 \\
c & 109 & 2017-12-26 & 3281.2358 & 0.0177 \\
b & 165 & 2018-01-01 & 3287.3218 & 0.0055 \\
c & 110 & 2018-01-07 & 3293.1563 & 0.0212 \\
b & 166 & 2018-01-09 & 3295.2385 & 0.0061 \\
b & 167 & 2018-01-17 & 3303.1587 & 0.0066 \\
c & 111 & 2018-01-19 & 3305.0661 & 0.0246 \\
b & 168 & 2018-01-25 & 3311.0756 & 0.0071 \\
c & 112 & 2018-01-31 & 3316.9873 & 0.0285 \\
b & 169 & 2018-02-02 & 3318.9925 & 0.0078 \\
b & 170 & 2018-02-10 & 3326.9128 & 0.0085 \\
c & 113 & 2018-02-12 & 3328.8975 & 0.0325 \\
b & 171 & 2018-02-18 & 3334.8298 & 0.0091 \\
c & 114 & 2018-02-24 & 3340.8188 & 0.0368 \\
b & 172 & 2018-02-26 & 3342.7463 & 0.0099 \\
b & 173 & 2018-03-06 & 3350.6663 & 0.0107 \\
c & 115 & 2018-03-08 & 3352.7289 & 0.0414 \\
b & 174 & 2018-03-14 & 3358.5834 & 0.0113 \\
c & 116 & 2018-03-20 & 3364.6496 & 0.0459 \\
b & 175 & 2018-03-22 & 3366.5003 & 0.0121 \\
b & 176 & 2018-03-29 & 3374.4207 & 0.0131 \\
c & 117 & 2018-04-01 & 3376.5589 & 0.0511 \\
b & 177 & 2018-04-06 & 3382.3381 & 0.0137 \\
c & 118 & 2018-04-12 & 3388.4785 & 0.0559 \\
b & 178 & 2018-04-14 & 3390.2549 & 0.0147 \\
b & 179 & 2018-04-22 & 3398.1751 & 0.0157 \\
c & 119 & 2018-04-24 & 3400.3866 & 0.0615 \\
b & 180 & 2018-04-30 & 3406.0927 & 0.0164 \\
c & 120 & 2018-05-06 & 3412.3045 & 0.0664 \\
b & 181 & 2018-05-08 & 3414.0100 & 0.0173 \\
b & 182 & 2018-05-16 & 3421.9308 & 0.0184 \\
c & 121 & 2018-05-18 & 3424.2107 & 0.0723 \\
b & 183 & 2018-05-24 & 3429.8490 & 0.0191 \\
c & 122 & 2018-05-30 & 3436.1263 & 0.0772 \\
b & 184 & 2018-06-01 & 3437.7665 & 0.0200 \\
b & 185 & 2018-06-09 & 3445.6874 & 0.0212 \\
c & 123 & 2018-06-11 & 3448.0303 & 0.0831 \\
b & 186 & 2018-06-17 & 3453.6058 & 0.0218 \\
c & 124 & 2018-06-23 & 3459.9433 & 0.0879 \\
b & 187 & 2018-06-25 & 3461.5238 & 0.0227 \\
b & 188 & 2018-07-02 & 3469.4454 & 0.0239 \\
c & 125 & 2018-07-05 & 3471.8445 & 0.0936 \\
b & 189 & 2018-07-10 & 3477.3647 & 0.0245 \\
c & 126 & 2018-07-17 & 3483.7543 & 0.0980 \\
b & 190 & 2018-07-18 & 3485.2832 & 0.0253 \\
b & 191 & 2018-07-26 & 3493.2050 & 0.0264 \\
c & 127 & 2018-07-29 & 3495.6526 & 0.1034 \\
b & 192 & 2018-08-03 & 3501.1245 & 0.0269 \\
c & 128 & 2018-08-10 & 3507.5591 & 0.1072 \\
b & 193 & 2018-08-11 & 3509.0435 & 0.0276 \\
b & 194 & 2018-08-19 & 3516.9661 & 0.0287 \\
c & 129 & 2018-08-21 & 3519.4541 & 0.1120 \\
b & 195 & 2018-08-27 & 3524.8866 & 0.0290 \\
c & 130 & 2018-09-02 & 3531.3570 & 0.1150 \\
b & 196 & 2018-09-04 & 3532.8062 & 0.0297 \\
b & 197 & 2018-09-12 & 3540.7292 & 0.0306 \\
c & 131 & 2018-09-14 & 3543.2488 & 0.1191 \\
b & 198 & 2018-09-20 & 3548.6500 & 0.0308 \\
c & 132 & 2018-09-26 & 3555.1482 & 0.1213 \\
b & 199 & 2018-09-28 & 3556.5699 & 0.0312 \\
b & 200 & 2018-10-05 & 3564.4936 & 0.0320 \\
c & 133 & 2018-10-08 & 3567.0366 & 0.1244 \\
b & 201 & 2018-10-13 & 3572.4154 & 0.0321 \\
c & 134 & 2018-10-20 & 3578.9325 & 0.1256 \\
b & 202 & 2018-10-21 & 3580.3361 & 0.0324 \\
b & 203 & 2018-10-29 & 3588.2602 & 0.0330 \\
c & 135 & 2018-11-01 & 3590.8179 & 0.1277 \\
b & 204 & 2018-11-06 & 3596.1822 & 0.0329 \\
c & 136 & 2018-11-13 & 3602.7106 & 0.1278 \\
b & 205 & 2018-11-14 & 3604.1032 & 0.0330 \\
b & 206 & 2018-11-22 & 3612.0278 & 0.0334 \\
c & 137 & 2018-11-25 & 3614.5932 & 0.1289 \\
b & 207 & 2018-11-30 & 3619.9506 & 0.0331 \\
c & 138 & 2018-12-06 & 3626.4831 & 0.1279 \\
b & 208 & 2018-12-08 & 3627.8723 & 0.0330 \\
b & 209 & 2018-12-16 & 3635.7973 & 0.0332 \\
c & 139 & 2018-12-18 & 3638.3633 & 0.1279 \\
b & 210 & 2018-12-24 & 3643.7203 & 0.0328 \\
c & 140 & 2018-12-30 & 3650.2509 & 0.1258 \\
b & 211 & 2019-01-01 & 3651.6420 & 0.0325 \\
b & 212 & 2019-01-09 & 3659.5673 & 0.0325 \\
c & 141 & 2019-01-11 & 3662.1291 & 0.1247 \\
b & 213 & 2019-01-16 & 3667.4909 & 0.0319 \\
c & 142 & 2019-01-23 & 3674.0150 & 0.1215 \\
b & 214 & 2019-01-24 & 3675.4132 & 0.0314 \\
b & 215 & 2019-02-01 & 3683.3387 & 0.0313 \\
c & 143 & 2019-02-04 & 3685.8920 & 0.1195 \\
b & 216 & 2019-02-09 & 3691.2623 & 0.0305 \\
c & 144 & 2019-02-16 & 3697.7767 & 0.1153 \\
b & 217 & 2019-02-17 & 3699.1845 & 0.0298 \\
b & 218 & 2019-02-25 & 3707.1100 & 0.0295 \\
c & 145 & 2019-02-28 & 3709.6531 & 0.1123 \\
b & 219 & 2019-03-05 & 3715.0338 & 0.0285 \\
c & 146 & 2019-03-12 & 3721.5375 & 0.1074 \\
b & 220 & 2019-03-13 & 3722.9565 & 0.0278 \\
b & 221 & 2019-03-21 & 3730.8821 & 0.0273 \\
c & 147 & 2019-03-23 & 3733.4139 & 0.1036 \\
b & 222 & 2019-03-29 & 3738.8057 & 0.0263 \\
c & 148 & 2019-04-04 & 3745.2985 & 0.0981 \\
b & 223 & 2019-04-06 & 3746.7280 & 0.0254 \\
b & 224 & 2019-04-14 & 3754.6532 & 0.0247 \\
c & 149 & 2019-04-16 & 3757.1757 & 0.0937 \\
b & 225 & 2019-04-22 & 3762.5768 & 0.0237 \\
c & 150 & 2019-04-28 & 3769.0613 & 0.0877 \\
b & 226 & 2019-04-29 & 3770.4993 & 0.0227 \\
b & 227 & 2019-05-07 & 3778.4245 & 0.0220 \\
c & 151 & 2019-05-10 & 3780.9400 & 0.0829 \\
b & 228 & 2019-05-15 & 3786.3478 & 0.0209 \\
c & 152 & 2019-05-22 & 3792.8271 & 0.0767 \\
b & 229 & 2019-05-23 & 3794.2696 & 0.0199 \\
b & 230 & 2019-05-31 & 3802.1942 & 0.0191 \\
c & 153 & 2019-06-03 & 3804.7079 & 0.0718 \\
b & 231 & 2019-06-08 & 3810.1171 & 0.0180 \\
c & 154 & 2019-06-15 & 3816.5973 & 0.0658 \\
b & 232 & 2019-06-16 & 3818.0389 & 0.0170 \\
b & 233 & 2019-06-24 & 3825.9633 & 0.0163 \\
c & 155 & 2019-06-26 & 3828.4808 & 0.0610 \\
b & 234 & 2019-07-02 & 3833.8858 & 0.0153 \\
c & 156 & 2019-07-08 & 3840.3728 & 0.0555 \\
b & 235 & 2019-07-10 & 3841.8069 & 0.0144 \\
b & 236 & 2019-07-18 & 3849.7304 & 0.0137 \\
c & 157 & 2019-07-20 & 3852.2595 & 0.0513 \\
b & 237 & 2019-07-26 & 3857.6523 & 0.0128 \\
c & 158 & 2019-08-01 & 3864.1546 & 0.0465 \\
b & 238 & 2019-08-03 & 3865.5731 & 0.0120 \\
b & 239 & 2019-08-10 & 3873.4963 & 0.0115 \\
c & 159 & 2019-08-13 & 3876.0448 & 0.0432 \\
b & 240 & 2019-08-18 & 3881.4178 & 0.0108 \\
c & 160 & 2019-08-25 & 3887.9431 & 0.0396 \\
b & 241 & 2019-08-26 & 3889.3379 & 0.0102 \\
b & 242 & 2019-09-03 & 3897.2600 & 0.0098 \\
c & 161 & 2019-09-06 & 3899.8371 & 0.0374 \\
b & 243 & 2019-09-11 & 3905.1808 & 0.0093 \\
c & 162 & 2019-09-18 & 3911.7389 & 0.0352 \\
b & 244 & 2019-09-19 & 3913.1005 & 0.0090 \\
b & 245 & 2019-09-27 & 3921.0223 & 0.0088 \\
c & 163 & 2019-09-30 & 3923.6367 & 0.0340 \\
b & 246 & 2019-10-05 & 3928.9427 & 0.0085 \\
c & 164 & 2019-10-12 & 3935.5417 & 0.0330 \\
b & 247 & 2019-10-13 & 3936.8617 & 0.0083 \\
b & 248 & 2019-10-21 & 3944.7825 & 0.0082 \\
c & 165 & 2019-10-23 & 3947.4433 & 0.0326 \\
b & 249 & 2019-10-29 & 3952.7022 & 0.0081 \\
c & 166 & 2019-11-04 & 3959.3515 & 0.0323 \\
b & 250 & 2019-11-06 & 3960.6207 & 0.0081 \\
b & 251 & 2019-11-14 & 3968.5412 & 0.0081 \\
c & 167 & 2019-11-16 & 3971.2565 & 0.0323 \\
b & 252 & 2019-11-21 & 3976.4608 & 0.0081 \\
c & 168 & 2019-11-28 & 3983.1674 & 0.0324 \\
b & 253 & 2019-11-29 & 3984.3788 & 0.0080 \\
b & 254 & 2019-12-07 & 3992.2984 & 0.0080 \\
c & 169 & 2019-12-10 & 3995.0755 & 0.0326 \\
b & 255 & 2019-12-15 & 4000.2174 & 0.0081 \\
c & 170 & 2019-12-22 & 4006.9887 & 0.0329 \\
b & 256 & 2019-12-23 & 4008.1349 & 0.0081 \\
b & 257 & 2019-12-31 & 4016.0542 & 0.0082 \\
c & 171 & 2020-01-03 & 4018.8993 & 0.0335 \\
b & 258 & 2020-01-08 & 4023.9733 & 0.0083 \\
c & 172 & 2020-01-15 & 4030.8143 & 0.0342 \\
b & 259 & 2020-01-16 & 4031.8906 & 0.0084 \\
b & 260 & 2020-01-24 & 4039.8094 & 0.0086 \\
c & 173 & 2020-01-27 & 4042.7269 & 0.0355 \\
b & 261 & 2020-02-01 & 4047.7280 & 0.0088 \\
c & 174 & 2020-02-08 & 4054.6429 & 0.0371 \\
b & 262 & 2020-02-09 & 4055.6449 & 0.0091 \\
b & 263 & 2020-02-17 & 4063.5635 & 0.0096 \\
c & 175 & 2020-02-20 & 4066.5568 & 0.0396 \\
b & 264 & 2020-02-24 & 4071.4824 & 0.0100 \\
c & 176 & 2020-03-02 & 4078.4734 & 0.0424 \\
b & 265 & 2020-03-03 & 4079.3995 & 0.0104 \\
b & 266 & 2020-03-11 & 4087.3179 & 0.0112 \\
c & 177 & 2020-03-14 & 4090.3878 & 0.0463 \\
b & 267 & 2020-03-19 & 4095.2366 & 0.0118 \\
c & 178 & 2020-03-26 & 4102.3044 & 0.0504 \\
b & 268 & 2020-03-27 & 4103.1533 & 0.0125 \\
b & 269 & 2020-04-04 & 4111.0717 & 0.0134 \\
c & 179 & 2020-04-07 & 4114.2188 & 0.0557 \\
b & 270 & 2020-04-12 & 4118.9908 & 0.0143 \\
c & 180 & 2020-04-19 & 4126.1347 & 0.0608 \\
b & 271 & 2020-04-20 & 4126.9080 & 0.0151 \\
b & 272 & 2020-04-28 & 4134.8264 & 0.0163 \\
c & 181 & 2020-05-01 & 4138.0484 & 0.0672 \\
b & 273 & 2020-05-06 & 4142.7456 & 0.0173 \\
c & 182 & 2020-05-13 & 4149.9632 & 0.0732 \\
b & 274 & 2020-05-14 & 4150.6626 & 0.0183 \\
b & 275 & 2020-05-22 & 4158.5811 & 0.0195 \\
c & 183 & 2020-05-25 & 4161.8757 & 0.0802 \\
b & 276 & 2020-05-30 & 4166.5008 & 0.0206 \\
c & 184 & 2020-06-06 & 4173.7889 & 0.0867 \\
b & 277 & 2020-06-06 & 4174.4184 & 0.0217 \\
b & 278 & 2020-06-14 & 4182.3372 & 0.0231 \\
c & 185 & 2020-06-18 & 4185.6998 & 0.0941 \\
b & 279 & 2020-06-22 & 4190.2571 & 0.0242 \\
c & 186 & 2020-06-30 & 4197.6111 & 0.1009 \\
b & 280 & 2020-06-30 & 4198.1748 & 0.0253 \\
b & 281 & 2020-07-08 & 4206.0937 & 0.0267 \\
c & 187 & 2020-07-12 & 4209.5201 & 0.1083 \\
b & 282 & 2020-07-16 & 4214.0141 & 0.0278 \\
c & 188 & 2020-07-23 & 4221.4292 & 0.1151 \\
b & 283 & 2020-07-24 & 4221.9325 & 0.0289 \\
b & 284 & 2020-08-01 & 4229.8519 & 0.0302 \\
c & 189 & 2020-08-04 & 4233.3360 & 0.1223 \\
b & 285 & 2020-08-09 & 4237.7727 & 0.0313 \\
c & 190 & 2020-08-16 & 4245.2427 & 0.1288 \\
b & 286 & 2020-08-17 & 4245.6913 & 0.0324 \\
b & 287 & 2020-08-25 & 4253.6107 & 0.0336 \\
c & 191 & 2020-08-28 & 4257.1472 & 0.1355 \\
b & 288 & 2020-09-02 & 4261.5320 & 0.0346 \\
c & 192 & 2020-09-09 & 4269.0515 & 0.1416 \\
b & 289 & 2020-09-09 & 4269.4512 & 0.0356 \\
b & 290 & 2020-09-17 & 4277.3713 & 0.0367 \\
c & 193 & 2020-09-21 & 4280.9537 & 0.1476 \\
b & 291 & 2020-09-25 & 4285.2930 & 0.0376 \\
c & 194 & 2020-10-03 & 4292.8557 & 0.1530 \\
b & 292 & 2020-10-03 & 4293.2125 & 0.0385 \\
b & 293 & 2020-10-11 & 4301.1326 & 0.0395 \\
c & 195 & 2020-10-15 & 4304.7557 & 0.1582 \\
b & 294 & 2020-10-19 & 4309.0546 & 0.0402 \\
c & 196 & 2020-10-27 & 4316.6555 & 0.1627 \\
b & 295 & 2020-10-27 & 4316.9746 & 0.0409 \\
b & 296 & 2020-11-04 & 4324.8954 & 0.0418 \\
c & 197 & 2020-11-08 & 4328.5534 & 0.1669 \\
b & 297 & 2020-11-12 & 4332.8178 & 0.0423 \\
c & 198 & 2020-11-19 & 4340.4512 & 0.1705 \\
b & 298 & 2020-11-20 & 4340.7381 & 0.0429 \\
b & 299 & 2020-11-28 & 4348.6588 & 0.0436 \\
c & 199 & 2020-12-01 & 4352.3474 & 0.1736 \\
b & 300 & 2020-12-06 & 4356.5814 & 0.0439 \\
c & 200 & 2020-12-13 & 4364.2433 & 0.1761 \\
b & 301 & 2020-12-14 & 4364.5022 & 0.0442 \\
b & 302 & 2020-12-21 & 4372.4234 & 0.0448 \\
c & 201 & 2020-12-25 & 4376.1381 & 0.1781 \\
b & 303 & 2020-12-29 & 4380.3464 & 0.0450 \\
c & 202 & 2021-01-06 & 4388.0327 & 0.1795 \\
b & 304 & 2021-01-06 & 4388.2673 & 0.0451 \\
b & 305 & 2021-01-14 & 4396.1885 & 0.0454 \\
c & 203 & 2021-01-18 & 4399.9265 & 0.1804 \\
b & 306 & 2021-01-22 & 4404.1114 & 0.0454 \\
c & 204 & 2021-01-30 & 4411.8200 & 0.1807 \\
b & 307 & 2021-01-30 & 4412.0325 & 0.0453 \\
b & 308 & 2021-02-07 & 4419.9541 & 0.0455 \\
c & 205 & 2021-02-11 & 4423.7131 & 0.1803 \\
b & 309 & 2021-02-15 & 4427.8774 & 0.0453 \\
c & 206 & 2021-02-23 & 4435.6061 & 0.1795 \\
b & 310 & 2021-02-23 & 4435.7986 & 0.0450 \\
b & 311 & 2021-03-03 & 4443.7199 & 0.0450 \\
c & 207 & 2021-03-06 & 4447.4990 & 0.1781 \\
b & 312 & 2021-03-11 & 4451.6430 & 0.0446 \\
c & 208 & 2021-03-18 & 4459.3917 & 0.1762 \\
b & 313 & 2021-03-19 & 4459.5642 & 0.0441 \\
b & 314 & 2021-03-26 & 4467.4857 & 0.0439 \\
c & 209 & 2021-03-30 & 4471.2849 & 0.1738 \\
b & 315 & 2021-04-03 & 4475.4090 & 0.0434 \\
c & 210 & 2021-04-11 & 4483.1779 & 0.1710 \\
b & 316 & 2021-04-11 & 4483.3302 & 0.0428 \\
b & 317 & 2021-04-19 & 4491.2515 & 0.0424 \\
c & 211 & 2021-04-23 & 4495.0717 & 0.1677 \\
b & 318 & 2021-04-27 & 4499.1744 & 0.0418 \\
c & 212 & 2021-05-05 & 4506.9654 & 0.1640 \\
b & 319 & 2021-05-05 & 4507.0954 & 0.0410 \\
b & 320 & 2021-05-13 & 4515.0166 & 0.0404 \\
c & 213 & 2021-05-17 & 4518.8603 & 0.1599 \\
b & 321 & 2021-05-21 & 4522.9396 & 0.0397 \\
c & 214 & 2021-05-29 & 4530.7550 & 0.1556 \\
b & 322 & 2021-05-29 & 4530.8606 & 0.0388 \\
b & 323 & 2021-06-06 & 4538.7814 & 0.0382 \\
c & 215 & 2021-06-10 & 4542.6513 & 0.1509 \\
b & 324 & 2021-06-14 & 4546.7039 & 0.0374 \\
c & 216 & 2021-06-22 & 4554.5475 & 0.1461 \\
b & 325 & 2021-06-22 & 4554.6245 & 0.0364 \\
b & 326 & 2021-06-30 & 4562.5450 & 0.0356 \\
c & 217 & 2021-07-03 & 4566.4456 & 0.1411 \\
b & 327 & 2021-07-07 & 4570.4676 & 0.0348 \\
c & 218 & 2021-07-15 & 4578.3435 & 0.1359 \\
b & 328 & 2021-07-15 & 4578.3880 & 0.0338 \\
b & 329 & 2021-07-23 & 4586.3082 & 0.0330 \\
c & 219 & 2021-07-27 & 4590.2436 & 0.1308 \\
b & 330 & 2021-07-31 & 4594.2302 & 0.0321 \\
c & 220 & 2021-08-08 & 4602.1436 & 0.1256 \\
b & 331 & 2021-08-08 & 4602.1501 & 0.0311 \\
b & 332 & 2021-08-16 & 4610.0698 & 0.0303 \\
c & 221 & 2021-08-20 & 4614.0459 & 0.1206 \\
b & 333 & 2021-08-24 & 4617.9917 & 0.0295 \\
b & 334 & 2021-09-01 & 4625.9114 & 0.0286 \\
c & 222 & 2021-09-01 & 4625.9481 & 0.1157 \\
b & 335 & 2021-09-09 & 4633.8308 & 0.0278 \\
c & 223 & 2021-09-13 & 4637.8528 & 0.1111 \\
b & 336 & 2021-09-17 & 4641.7521 & 0.0271 \\
b & 337 & 2021-09-25 & 4649.6712 & 0.0262 \\
c & 224 & 2021-09-25 & 4649.7573 & 0.1065 \\
b & 338 & 2021-10-03 & 4657.5900 & 0.0256 \\
c & 225 & 2021-10-07 & 4661.6645 & 0.1026 \\
b & 339 & 2021-10-11 & 4665.5110 & 0.0250 \\
b & 340 & 2021-10-18 & 4673.4301 & 0.0242 \\
c & 226 & 2021-10-19 & 4673.5714 & 0.0988 \\
b & 341 & 2021-10-26 & 4681.3486 & 0.0237 \\
c & 227 & 2021-10-30 & 4685.4810 & 0.0957 \\
b & 342 & 2021-11-03 & 4689.2691 & 0.0233 \\
b & 343 & 2021-11-11 & 4697.1875 & 0.0227 \\
c & 228 & 2021-11-11 & 4697.3904 & 0.0928 \\
b & 344 & 2021-11-19 & 4705.1053 & 0.0223 \\
c & 229 & 2021-11-23 & 4709.3022 & 0.0907 \\
b & 345 & 2021-11-27 & 4713.0255 & 0.0220 \\
b & 346 & 2021-12-05 & 4720.9439 & 0.0216 \\
c & 230 & 2021-12-05 & 4721.2139 & 0.0888 \\
b & 347 & 2021-12-13 & 4728.8615 & 0.0215 \\
c & 231 & 2021-12-17 & 4733.1279 & 0.0878 \\
b & 348 & 2021-12-21 & 4736.7813 & 0.0213 \\
b & 349 & 2021-12-29 & 4744.6990 & 0.0211 \\
c & 232 & 2021-12-29 & 4745.0418 & 0.0869 \\
b & 350 & 2022-01-06 & 4752.6161 & 0.0211 \\
c & 233 & 2022-01-10 & 4756.9578 & 0.0870 \\
b & 351 & 2022-01-14 & 4760.5355 & 0.0212 \\
b & 352 & 2022-01-21 & 4768.4532 & 0.0211 \\
c & 234 & 2022-01-22 & 4768.8734 & 0.0870 \\
b & 353 & 2022-01-29 & 4776.3702 & 0.0213 \\
c & 235 & 2022-02-03 & 4780.7911 & 0.0881 \\
b & 354 & 2022-02-06 & 4784.2893 & 0.0216 \\
b & 355 & 2022-02-14 & 4792.2067 & 0.0216 \\
c & 236 & 2022-02-15 & 4792.7083 & 0.0890 \\
b & 356 & 2022-02-22 & 4800.1231 & 0.0220 \\
c & 237 & 2022-02-27 & 4804.6273 & 0.0911 \\
b & 357 & 2022-03-02 & 4808.0418 & 0.0224 \\
b & 358 & 2022-03-10 & 4815.9593 & 0.0226 \\
c & 238 & 2022-03-11 & 4816.5455 & 0.0928 \\
b & 359 & 2022-03-18 & 4823.8758 & 0.0231 \\
c & 239 & 2022-03-22 & 4828.4655 & 0.0957 \\
b & 360 & 2022-03-26 & 4831.7945 & 0.0237 \\
b & 361 & 2022-04-03 & 4839.7118 & 0.0240 \\
c & 240 & 2022-04-03 & 4840.3843 & 0.0983 \\
b & 362 & 2022-04-11 & 4847.6279 & 0.0247 \\
c & 241 & 2022-04-15 & 4852.3048 & 0.1021 \\
b & 363 & 2022-04-19 & 4855.5462 & 0.0254 \\
b & 364 & 2022-04-26 & 4863.4637 & 0.0258 \\
c & 242 & 2022-04-27 & 4864.2236 & 0.1053 \\
b & 365 & 2022-05-04 & 4871.3801 & 0.0266 \\
c & 243 & 2022-05-09 & 4876.1441 & 0.1100 \\
b & 366 & 2022-05-12 & 4879.2985 & 0.0275 \\
b & 367 & 2022-05-20 & 4887.2161 & 0.0281 \\
c & 244 & 2022-05-21 & 4888.0624 & 0.1139 \\
b & 368 & 2022-05-28 & 4895.1324 & 0.0290 \\
c & 245 & 2022-06-02 & 4899.9824 & 0.1194 \\
b & 369 & 2022-06-05 & 4903.0506 & 0.0300 \\
b & 370 & 2022-06-13 & 4910.9684 & 0.0307 \\
c & 246 & 2022-06-14 & 4911.8996 & 0.1239 \\
b & 371 & 2022-06-21 & 4918.8851 & 0.0317 \\
c & 247 & 2022-06-26 & 4923.8184 & 0.1301 \\
b & 372 & 2022-06-29 & 4926.8037 & 0.0329 \\
b & 373 & 2022-07-07 & 4934.7219 & 0.0336 \\
c & 248 & 2022-07-08 & 4935.7338 & 0.1351 \\
b & 374 & 2022-07-15 & 4942.6387 & 0.0347 \\
c & 249 & 2022-07-20 & 4947.6511 & 0.1417 \\
b & 375 & 2022-07-23 & 4950.5572 & 0.0360 \\
b & 376 & 2022-07-30 & 4958.4758 & 0.0367 \\
c & 250 & 2022-08-01 & 4959.5641 & 0.1469 \\
b & 377 & 2022-08-07 & 4966.3932 & 0.0378 \\
c & 251 & 2022-08-12 & 4971.4791 & 0.1537 \\
b & 378 & 2022-08-15 & 4974.3122 & 0.0392 \\
b & 379 & 2022-08-23 & 4982.2316 & 0.0399 \\
c & 252 & 2022-08-24 & 4983.3891 & 0.1588 \\
b & 380 & 2022-08-31 & 4990.1493 & 0.0409 \\
c & 253 & 2022-09-05 & 4995.3014 & 0.1655 \\
b & 381 & 2022-09-08 & 4998.0685 & 0.0423 \\
b & 382 & 2022-09-16 & 5005.9883 & 0.0429 \\
c & 254 & 2022-09-17 & 5007.2079 & 0.1702 \\
b & 383 & 2022-09-24 & 5013.9066 & 0.0439 \\
c & 255 & 2022-09-29 & 5019.1170 & 0.1763 \\
b & 384 & 2022-10-02 & 5021.8266 & 0.0451 \\
b & 385 & 2022-10-10 & 5029.7474 & 0.0456 \\
c & 256 & 2022-10-11 & 5031.0196 & 0.1802 \\
b & 386 & 2022-10-18 & 5037.6663 & 0.0464 \\
c & 257 & 2022-10-23 & 5042.9252 & 0.1855 \\
b & 387 & 2022-10-26 & 5045.5865 & 0.0476 \\
b & 388 & 2022-11-03 & 5053.5078 & 0.0478 \\
c & 258 & 2022-11-04 & 5054.8235 & 0.1881 \\
b & 389 & 2022-11-10 & 5061.4273 & 0.0484 \\
c & 259 & 2022-11-16 & 5066.7253 & 0.1922 \\
b & 390 & 2022-11-18 & 5069.3484 & 0.0493 \\
b & 391 & 2022-11-26 & 5077.2707 & 0.0493 \\
c & 260 & 2022-11-28 & 5078.6193 & 0.1934 \\
b & 392 & 2022-12-04 & 5085.1910 & 0.0496 \\
c & 261 & 2022-12-10 & 5090.5173 & 0.1959 \\
b & 393 & 2022-12-12 & 5093.1125 & 0.0504 \\
b & 394 & 2022-12-20 & 5101.0353 & 0.0501 \\
c & 262 & 2022-12-21 & 5102.4071 & 0.1954 \\
b & 395 & 2022-12-28 & 5108.9561 & 0.0501 \\
c & 263 & 2023-01-02 & 5114.3013 & 0.1962 \\
b & 396 & 2023-01-05 & 5116.8784 & 0.0505 \\
b & 397 & 2023-01-13 & 5124.8021 & 0.0499 \\
c & 264 & 2023-01-14 & 5126.1872 & 0.1938 \\
b & 398 & 2023-01-21 & 5132.7237 & 0.0496 \\
c & 265 & 2023-01-26 & 5138.0779 & 0.1928 \\
b & 399 & 2023-01-29 & 5140.6464 & 0.0497 \\
b & 400 & 2023-02-06 & 5148.5705 & 0.0488 \\
c & 266 & 2023-02-07 & 5149.9603 & 0.1886 \\
b & 401 & 2023-02-13 & 5156.4923 & 0.0481 \\
c & 267 & 2023-02-19 & 5161.8480 & 0.1857 \\
b & 402 & 2023-02-21 & 5164.4157 & 0.0479 \\
b & 403 & 2023-03-01 & 5172.3406 & 0.0467 \\
c & 268 & 2023-03-03 & 5173.7275 & 0.1798 \\
b & 404 & 2023-03-09 & 5180.2630 & 0.0458 \\
c & 269 & 2023-03-15 & 5185.6127 & 0.1751 \\
b & 405 & 2023-03-17 & 5188.1867 & 0.0453 \\
b & 406 & 2023-03-25 & 5196.1118 & 0.0438 \\
c & 270 & 2023-03-26 & 5197.4899 & 0.1676 \\
b & 407 & 2023-04-02 & 5204.0342 & 0.0426 \\
c & 271 & 2023-04-07 & 5209.3735 & 0.1613 \\
b & 408 & 2023-04-10 & 5211.9582 & 0.0418 \\
b & 409 & 2023-04-18 & 5219.8837 & 0.0401 \\
c & 272 & 2023-04-19 & 5221.2492 & 0.1524 \\
b & 410 & 2023-04-26 & 5227.8067 & 0.0387 \\
c & 273 & 2023-05-01 & 5233.1318 & 0.1448 \\
b & 411 & 2023-05-04 & 5235.7308 & 0.0376 \\
b & 412 & 2023-05-12 & 5243.6563 & 0.0358 \\
c & 274 & 2023-05-13 & 5245.0069 & 0.1350 \\
b & 413 & 2023-05-20 & 5251.5790 & 0.0342 \\
c & 275 & 2023-05-25 & 5256.8893 & 0.1264 \\
b & 414 & 2023-05-28 & 5259.5031 & 0.0330 \\
b & 415 & 2023-06-04 & 5267.4287 & 0.0310 \\
c & 276 & 2023-06-06 & 5268.7645 & 0.1159 \\
b & 416 & 2023-06-12 & 5275.3515 & 0.0294 \\
c & 277 & 2023-06-18 & 5280.6476 & 0.1068 \\
b & 417 & 2023-06-20 & 5283.2756 & 0.0281 \\
b & 418 & 2023-06-28 & 5291.2010 & 0.0261 \\
c & 278 & 2023-06-30 & 5292.5237 & 0.0961 \\
b & 419 & 2023-07-06 & 5299.1233 & 0.0244 \\
c & 279 & 2023-07-11 & 5304.4082 & 0.0870 \\
b & 420 & 2023-07-14 & 5307.0470 & 0.0231 \\
b & 421 & 2023-07-22 & 5314.9721 & 0.0211 \\
c & 280 & 2023-07-23 & 5316.2860 & 0.0767 \\
b & 422 & 2023-07-30 & 5322.8944 & 0.0196 \\
c & 281 & 2023-08-04 & 5328.1727 & 0.0682 \\
b & 423 & 2023-08-07 & 5330.8179 & 0.0183 \\
b & 424 & 2023-08-15 & 5338.7426 & 0.0166 \\
c & 282 & 2023-08-16 & 5340.0527 & 0.0590 \\
b & 425 & 2023-08-23 & 5346.6641 & 0.0153 \\
c & 283 & 2023-08-28 & 5351.9422 & 0.0522 \\
b & 426 & 2023-08-31 & 5354.5869 & 0.0142 \\
b & 427 & 2023-09-08 & 5362.5112 & 0.0129 \\
c & 284 & 2023-09-09 & 5363.8251 & 0.0454 \\
b & 428 & 2023-09-15 & 5370.4324 & 0.0120 \\
c & 285 & 2023-09-21 & 5375.7178 & 0.0416 \\
b & 429 & 2023-09-23 & 5378.3549 & 0.0114 \\
b & 430 & 2023-10-01 & 5386.2787 & 0.0106 \\
c & 286 & 2023-10-03 & 5387.6039 & 0.0386 \\
b & 431 & 2023-10-09 & 5394.1991 & 0.0103 \\
c & 287 & 2023-10-15 & 5399.5002 & 0.0387 \\
b & 432 & 2023-10-17 & 5402.1207 & 0.0103 \\
b & 433 & 2023-10-25 & 5410.0438 & 0.0103 \\
c & 288 & 2023-10-26 & 5411.3898 & 0.0396 \\
b & 434 & 2023-11-02 & 5417.9637 & 0.0105 \\
c & 289 & 2023-11-07 & 5423.2900 & 0.0424 \\
b & 435 & 2023-11-10 & 5425.8850 & 0.0109 \\
b & 436 & 2023-11-18 & 5433.8076 & 0.0111 \\
c & 290 & 2023-11-19 & 5435.1831 & 0.0452 \\
b & 437 & 2023-11-26 & 5441.7268 & 0.0115 \\
c & 291 & 2023-12-01 & 5447.0871 & 0.0487 \\
b & 438 & 2023-12-04 & 5449.6471 & 0.0121 \\
b & 439 & 2023-12-12 & 5457.5690 & 0.0125 \\
c & 292 & 2023-12-13 & 5458.9837 & 0.0515 \\
b & 440 & 2023-12-19 & 5465.4877 & 0.0129 \\
c & 293 & 2023-12-25 & 5470.8912 & 0.0545 \\
b & 441 & 2023-12-27 & 5473.4076 & 0.0134 \\
b & 442 & 2024-01-04 & 5481.3293 & 0.0136 \\
c & 294 & 2024-01-06 & 5482.7910 & 0.0565 \\
b & 443 & 2024-01-12 & 5489.2474 & 0.0138 \\
c & 295 & 2024-01-18 & 5494.7018 & 0.0584 \\
b & 444 & 2024-01-20 & 5497.1664 & 0.0141 \\
b & 445 & 2024-01-28 & 5505.0874 & 0.0143 \\
c & 296 & 2024-01-30 & 5506.6044 & 0.0593 \\
b & 446 & 2024-02-05 & 5513.0052 & 0.0144 \\
c & 297 & 2024-02-11 & 5518.5179 & 0.0602 \\
b & 447 & 2024-02-13 & 5520.9240 & 0.0146 \\
b & 448 & 2024-02-21 & 5528.8449 & 0.0145 \\
c & 298 & 2024-02-22 & 5530.4225 & 0.0600 \\
b & 449 & 2024-02-29 & 5536.7624 & 0.0144 \\
c & 299 & 2024-03-05 & 5542.3380 & 0.0601 \\
b & 450 & 2024-03-08 & 5544.6806 & 0.0144 \\
b & 451 & 2024-03-16 & 5552.6010 & 0.0143 \\
c & 300 & 2024-03-17 & 5554.2441 & 0.0592 \\
b & 452 & 2024-03-24 & 5560.5183 & 0.0143 \\
c & 301 & 2024-03-29 & 5566.1608 & 0.0592 \\
b & 453 & 2024-03-31 & 5568.4363 & 0.0143 \\
b & 454 & 2024-04-08 & 5576.3571 & 0.0142 \\
c & 302 & 2024-04-10 & 5578.0674 & 0.0583 \\
b & 455 & 2024-04-16 & 5584.2744 & 0.0142 \\
c & 303 & 2024-04-22 & 5589.9845 & 0.0589 \\
b & 456 & 2024-04-24 & 5592.1922 & 0.0144 \\
b & 457 & 2024-05-02 & 5600.1128 & 0.0145 \\
c & 304 & 2024-05-04 & 5601.8909 & 0.0590 \\
b & 458 & 2024-05-10 & 5608.0300 & 0.0148 \\
c & 305 & 2024-05-16 & 5613.8077 & 0.0611 \\
b & 459 & 2024-05-18 & 5615.9478 & 0.0153 \\
b & 460 & 2024-05-26 & 5623.8689 & 0.0157 \\
c & 306 & 2024-05-28 & 5625.7131 & 0.0631 \\
b & 461 & 2024-06-03 & 5631.7866 & 0.0163 \\
c & 307 & 2024-06-09 & 5637.6288 & 0.0671 \\
b & 462 & 2024-06-11 & 5639.7045 & 0.0172 \\
b & 463 & 2024-06-19 & 5647.6257 & 0.0180 \\
c & 308 & 2024-06-21 & 5649.5326 & 0.0713 \\
b & 464 & 2024-06-27 & 5655.5434 & 0.0189 \\
c & 309 & 2024-07-02 & 5661.4467 & 0.0771 \\
b & 465 & 2024-07-04 & 5663.4615 & 0.0201 \\
b & 466 & 2024-07-12 & 5671.3833 & 0.0212 \\
c & 310 & 2024-07-14 & 5673.3484 & 0.0831 \\
b & 467 & 2024-07-20 & 5679.3017 & 0.0223 \\
c & 311 & 2024-07-26 & 5685.2604 & 0.0902 \\
b & 468 & 2024-07-28 & 5687.2202 & 0.0237 \\
b & 469 & 2024-08-05 & 5695.1422 & 0.0250 \\
c & 312 & 2024-08-07 & 5697.1597 & 0.0975 \\
b & 470 & 2024-08-13 & 5703.0608 & 0.0262 \\
c & 313 & 2024-08-19 & 5709.0693 & 0.1054 \\
b & 471 & 2024-08-21 & 5710.9795 & 0.0278 \\
b & 472 & 2024-08-29 & 5718.9021 & 0.0292 \\
c & 314 & 2024-08-31 & 5720.9660 & 0.1133 \\
b & 473 & 2024-09-06 & 5726.8214 & 0.0304 \\
c & 315 & 2024-09-12 & 5732.8730 & 0.1215 \\
b & 474 & 2024-09-14 & 5734.7406 & 0.0320 \\
b & 475 & 2024-09-22 & 5742.6636 & 0.0335 \\
c & 316 & 2024-09-24 & 5744.7672 & 0.1296 \\
b & 476 & 2024-09-30 & 5750.5832 & 0.0346 \\
c & 317 & 2024-10-06 & 5756.6716 & 0.1376 \\
b & 477 & 2024-10-08 & 5758.5026 & 0.0362 \\
b & 478 & 2024-10-15 & 5766.4260 & 0.0376 \\
c & 318 & 2024-10-18 & 5768.5632 & 0.1456 \\
b & 479 & 2024-10-23 & 5774.3463 & 0.0387 \\
c & 319 & 2024-10-29 & 5780.4651 & 0.1530 \\
b & 480 & 2024-10-31 & 5782.2663 & 0.0402 \\
b & 481 & 2024-11-08 & 5790.1901 & 0.0415 \\
c & 320 & 2024-11-10 & 5792.3544 & 0.1604 \\
b & 482 & 2024-11-16 & 5798.1106 & 0.0425 \\
c & 321 & 2024-11-22 & 5804.2540 & 0.1670 \\
b & 483 & 2024-11-24 & 5806.0307 & 0.0438 \\
b & 484 & 2024-12-02 & 5813.9548 & 0.0450 \\
c & 322 & 2024-12-04 & 5816.1411 & 0.1737 \\
b & 485 & 2024-12-10 & 5821.8760 & 0.0457 \\
c & 323 & 2024-12-16 & 5828.0386 & 0.1791 \\
b & 486 & 2024-12-18 & 5829.7967 & 0.0469 \\
b & 487 & 2024-12-26 & 5837.7211 & 0.0480 \\
c & 324 & 2024-12-28 & 5839.9240 & 0.1847 \\
b & 488 & 2025-01-03 & 5845.6424 & 0.0484 \\
c & 325 & 2025-01-09 & 5851.8197 & 0.1889 \\
b & 489 & 2025-01-11 & 5853.5631 & 0.0494 \\
b & 490 & 2025-01-18 & 5861.4876 & 0.0502 \\
c & 326 & 2025-01-21 & 5863.7036 & 0.1933 \\
b & 491 & 2025-01-26 & 5869.4093 & 0.0505 \\
c & 327 & 2025-02-02 & 5875.5980 & 0.1960 \\
b & 492 & 2025-02-03 & 5877.3305 & 0.0512 \\
b & 493 & 2025-02-11 & 5885.2553 & 0.0518 \\
c & 328 & 2025-02-13 & 5887.4809 & 0.1991 \\
b & 494 & 2025-02-19 & 5893.1771 & 0.0518 \\
c & 329 & 2025-02-25 & 5899.3743 & 0.2002 \\
b & 495 & 2025-02-27 & 5901.0982 & 0.0522 \\
b & 496 & 2025-03-07 & 5909.0230 & 0.0526 \\
c & 330 & 2025-03-09 & 5911.2565 & 0.2019 \\
b & 497 & 2025-03-15 & 5916.9449 & 0.0523 \\
c & 331 & 2025-03-21 & 5923.1494 & 0.2015 \\
b & 498 & 2025-03-23 & 5924.8664 & 0.0525 \\
b & 499 & 2025-03-31 & 5932.7913 & 0.0527 \\
c & 332 & 2025-04-02 & 5935.0315 & 0.2017 \\
b & 500 & 2025-04-08 & 5940.7133 & 0.0521 \\
c & 333 & 2025-04-14 & 5946.9243 & 0.1997 \\
b & 501 & 2025-04-16 & 5948.6345 & 0.0520 \\
b & 502 & 2025-04-24 & 5956.5591 & 0.0519 \\
c & 334 & 2025-04-26 & 5958.8067 & 0.1985 \\
b & 503 & 2025-05-01 & 5964.4810 & 0.0511 \\
c & 335 & 2025-05-08 & 5970.6998 & 0.1952 \\
b & 504 & 2025-05-09 & 5972.4024 & 0.0508 \\
b & 505 & 2025-05-17 & 5980.3271 & 0.0505 \\
c & 336 & 2025-05-20 & 5982.5829 & 0.1927 \\
b & 506 & 2025-05-25 & 5988.2490 & 0.0495 \\
c & 337 & 2025-05-31 & 5994.4768 & 0.1881 \\
b & 507 & 2025-06-02 & 5996.1700 & 0.0489 \\
b & 508 & 2025-06-10 & 6004.0943 & 0.0485 \\
c & 338 & 2025-06-12 & 6006.3611 & 0.1845 \\
b & 509 & 2025-06-18 & 6012.0159 & 0.0473 \\
c & 339 & 2025-06-24 & 6018.2561 & 0.1789 \\
b & 510 & 2025-06-26 & 6019.9369 & 0.0465 \\
b & 511 & 2025-07-04 & 6027.8611 & 0.0459 \\
c & 340 & 2025-07-06 & 6030.1419 & 0.1744 \\
b & 512 & 2025-07-12 & 6035.7826 & 0.0446 \\
c & 341 & 2025-07-18 & 6042.0384 & 0.1681 \\
b & 513 & 2025-07-20 & 6043.7032 & 0.0437 \\
b & 514 & 2025-07-28 & 6051.6269 & 0.0430 \\
c & 342 & 2025-07-30 & 6053.9261 & 0.1631 \\
b & 515 & 2025-08-05 & 6059.5479 & 0.0416 \\
c & 343 & 2025-08-11 & 6065.8243 & 0.1564 \\
b & 516 & 2025-08-12 & 6067.4683 & 0.0406 \\
b & 517 & 2025-08-20 & 6075.3918 & 0.0399 \\
c & 344 & 2025-08-23 & 6077.7141 & 0.1512 \\
b & 518 & 2025-08-28 & 6083.3128 & 0.0385 \\
c & 345 & 2025-09-04 & 6089.6142 & 0.1446 \\
b & 519 & 2025-09-05 & 6091.2328 & 0.0375 \\
b & 520 & 2025-09-13 & 6099.1557 & 0.0368 \\
c & 346 & 2025-09-16 & 6101.5064 & 0.1397 \\
b & 521 & 2025-09-21 & 6107.0761 & 0.0355 \\
c & 347 & 2025-09-27 & 6113.4086 & 0.1336 \\
b & 522 & 2025-09-29 & 6114.9957 & 0.0346 \\
b & 523 & 2025-10-07 & 6122.9183 & 0.0340 \\
c & 348 & 2025-10-09 & 6125.3032 & 0.1293 \\
b & 524 & 2025-10-15 & 6130.8386 & 0.0329 \\
c & 349 & 2025-10-21 & 6137.2074 & 0.1241 \\
b & 525 & 2025-10-23 & 6138.7579 & 0.0321 \\
b & 526 & 2025-10-31 & 6146.6799 & 0.0316 \\
c & 350 & 2025-11-02 & 6149.1046 & 0.1209 \\
b & 527 & 2025-11-08 & 6154.5997 & 0.0307 \\
c & 351 & 2025-11-14 & 6161.0107 & 0.1170 \\
b & 528 & 2025-11-16 & 6162.5185 & 0.0301 \\
b & 529 & 2025-11-23 & 6170.4402 & 0.0299 \\
c & 352 & 2025-11-26 & 6172.9103 & 0.1151 \\
b & 530 & 2025-12-01 & 6178.3600 & 0.0292 \\
c & 353 & 2025-12-08 & 6184.8183 & 0.1126 \\
b & 531 & 2025-12-09 & 6186.2786 & 0.0288 \\
b & 532 & 2025-12-17 & 6194.1998 & 0.0288 \\
c & 354 & 2025-12-20 & 6196.7201 & 0.1121 \\
b & 533 & 2025-12-25 & 6202.1191 & 0.0284 \\
c & 355 & 2026-01-01 & 6208.6297 & 0.1110 \\
b & 534 & 2026-01-02 & 6210.0373 & 0.0282 \\
b & 535 & 2026-01-10 & 6217.9581 & 0.0285 \\
c & 356 & 2026-01-13 & 6220.5334 & 0.1119 \\
b & 536 & 2026-01-18 & 6225.8775 & 0.0283 \\
c & 357 & 2026-01-24 & 6232.4443 & 0.1119 \\
b & 537 & 2026-01-26 & 6233.7956 & 0.0283 \\
b & 538 & 2026-02-03 & 6241.7160 & 0.0288 \\
c & 358 & 2026-02-05 & 6244.3497 & 0.1137 \\
b & 539 & 2026-02-11 & 6249.6352 & 0.0287 \\
c & 359 & 2026-02-17 & 6256.2615 & 0.1146 \\
b & 540 & 2026-02-19 & 6257.5528 & 0.0289 \\
b & 541 & 2026-02-26 & 6265.4730 & 0.0295 \\
c & 360 & 2026-03-01 & 6268.1681 & 0.1172 \\
b & 542 & 2026-03-06 & 6273.3923 & 0.0296 \\
c & 361 & 2026-03-13 & 6280.0804 & 0.1186 \\
b & 543 & 2026-03-14 & 6281.3101 & 0.0299 \\
b & 544 & 2026-03-22 & 6289.2300 & 0.0306 \\
c & 362 & 2026-03-25 & 6291.9879 & 0.1217 \\
b & 545 & 2026-03-30 & 6297.1493 & 0.0307 \\
c & 363 & 2026-04-06 & 6303.9002 & 0.1235 \\
b & 546 & 2026-04-07 & 6305.0668 & 0.0311 \\
b & 547 & 2026-04-15 & 6312.9865 & 0.0319 \\
c & 364 & 2026-04-18 & 6315.8079 & 0.1270 \\
b & 548 & 2026-04-23 & 6320.9060 & 0.0321 \\
c & 365 & 2026-04-30 & 6327.7199 & 0.1292 \\
b & 549 & 2026-05-01 & 6328.8238 & 0.0326 \\
b & 550 & 2026-05-09 & 6336.7436 & 0.0335 \\
c & 366 & 2026-05-12 & 6339.6275 & 0.1332 \\
b & 551 & 2026-05-17 & 6344.6632 & 0.0338 \\
c & 367 & 2026-05-24 & 6351.5386 & 0.1358 \\
b & 552 & 2026-05-25 & 6352.5810 & 0.0343 \\
b & 553 & 2026-06-02 & 6360.5006 & 0.0353 \\
c & 368 & 2026-06-04 & 6363.4456 & 0.1403 \\
b & 554 & 2026-06-09 & 6368.4205 & 0.0357 \\
c & 369 & 2026-06-16 & 6375.3557 & 0.1434 \\
b & 555 & 2026-06-17 & 6376.3387 & 0.0363 \\
b & 556 & 2026-06-25 & 6384.2586 & 0.0375 \\
c & 370 & 2026-06-28 & 6387.2617 & 0.1486 \\
b & 557 & 2026-07-03 & 6392.1788 & 0.0379 \\
c & 371 & 2026-07-10 & 6399.1702 & 0.1524 \\
b & 558 & 2026-07-11 & 6400.0970 & 0.0387 \\
b & 559 & 2026-07-19 & 6408.0169 & 0.0400 \\
c & 372 & 2026-07-22 & 6411.0749 & 0.1583 \\
b & 560 & 2026-07-27 & 6415.9373 & 0.0405 \\
c & 373 & 2026-08-03 & 6422.9817 & 0.1628 \\
b & 561 & 2026-08-04 & 6423.8560 & 0.0413 \\
b & 562 & 2026-08-12 & 6431.7764 & 0.0428 \\
c & 374 & 2026-08-15 & 6434.8848 & 0.1694 \\
b & 563 & 2026-08-20 & 6439.6973 & 0.0434 \\
c & 375 & 2026-08-27 & 6446.7897 & 0.1745 \\
b & 564 & 2026-08-28 & 6447.6162 & 0.0444 \\
b & 565 & 2026-09-05 & 6455.5365 & 0.0459 \\
c & 376 & 2026-09-08 & 6458.6910 & 0.1817 \\
b & 566 & 2026-09-12 & 6463.4577 & 0.0466 \\
c & 377 & 2026-09-20 & 6470.5939 & 0.1872 \\
b & 567 & 2026-09-20 & 6471.3770 & 0.0476 \\
b & 568 & 2026-09-28 & 6479.2979 & 0.0492 \\
c & 378 & 2026-10-01 & 6482.4935 & 0.1948 \\
b & 569 & 2026-10-06 & 6487.2195 & 0.0500 \\
c & 379 & 2026-10-13 & 6494.3943 & 0.2006 \\
b & 570 & 2026-10-14 & 6495.1391 & 0.0510 \\
b & 571 & 2026-10-22 & 6503.0601 & 0.0526 \\
c & 380 & 2026-10-25 & 6506.2921 & 0.2083 \\
b & 572 & 2026-10-30 & 6510.9819 & 0.0534 \\
c & 381 & 2026-11-06 & 6518.1910 & 0.2141 \\
b & 573 & 2026-11-07 & 6518.9019 & 0.0543 \\
b & 574 & 2026-11-15 & 6526.8233 & 0.0559 \\
c & 382 & 2026-11-18 & 6530.0871 & 0.2216 \\
b & 575 & 2026-11-23 & 6534.7456 & 0.0567 \\
c & 383 & 2026-11-30 & 6541.9842 & 0.2272 \\
b & 576 & 2026-12-01 & 6542.6659 & 0.0576 \\
b & 577 & 2026-12-09 & 6550.5874 & 0.0591 \\
c & 384 & 2026-12-12 & 6553.8788 & 0.2342 \\
b & 578 & 2026-12-17 & 6558.5098 & 0.0597 \\
c & 385 & 2026-12-24 & 6565.7744 & 0.2393 \\
b & 579 & 2026-12-24 & 6566.4304 & 0.0605 \\
b & 580 & 2027-01-01 & 6574.3522 & 0.0619 \\
c & 386 & 2027-01-05 & 6577.6678 & 0.2456 \\
b & 581 & 2027-01-09 & 6582.2750 & 0.0624 \\
c & 387 & 2027-01-17 & 6589.5620 & 0.2499 \\
b & 582 & 2027-01-17 & 6590.1958 & 0.0631 \\
b & 583 & 2027-01-25 & 6598.1177 & 0.0643 \\
c & 388 & 2027-01-28 & 6601.4545 & 0.2552 \\
b & 584 & 2027-02-02 & 6606.0404 & 0.0647 \\
c & 389 & 2027-02-09 & 6613.3479 & 0.2586 \\
b & 585 & 2027-02-10 & 6613.9613 & 0.0652 \\
b & 586 & 2027-02-18 & 6621.8834 & 0.0662 \\
c & 390 & 2027-02-21 & 6625.2398 & 0.2628 \\
b & 587 & 2027-02-26 & 6629.8065 & 0.0664 \\
c & 391 & 2027-03-05 & 6637.1326 & 0.2650 \\
b & 588 & 2027-03-06 & 6637.7276 & 0.0667 \\
b & 589 & 2027-03-14 & 6645.6495 & 0.0675 \\
c & 392 & 2027-03-17 & 6649.0244 & 0.2680 \\
b & 590 & 2027-03-22 & 6653.5725 & 0.0674 \\
c & 393 & 2027-03-29 & 6660.9171 & 0.2690 \\
b & 591 & 2027-03-29 & 6661.4935 & 0.0675 \\
b & 592 & 2027-04-06 & 6669.4154 & 0.0681 \\
c & 394 & 2027-04-10 & 6672.8091 & 0.2706 \\
b & 593 & 2027-04-14 & 6677.3385 & 0.0678 \\
c & 395 & 2027-04-22 & 6684.7020 & 0.2705 \\
b & 594 & 2027-04-22 & 6685.2596 & 0.0677 \\
b & 595 & 2027-04-30 & 6693.1814 & 0.0680 \\
c & 396 & 2027-05-04 & 6696.5948 & 0.2708 \\
b & 596 & 2027-05-08 & 6701.1043 & 0.0676 \\
c & 397 & 2027-05-15 & 6708.4883 & 0.2694 \\
b & 597 & 2027-05-16 & 6709.0251 & 0.0673 \\
b & 598 & 2027-05-24 & 6716.9467 & 0.0674 \\
c & 398 & 2027-05-27 & 6720.3820 & 0.2685 \\
b & 599 & 2027-06-01 & 6724.8696 & 0.0668 \\
c & 399 & 2027-06-08 & 6732.2765 & 0.2660 \\
b & 600 & 2027-06-09 & 6732.7904 & 0.0662 \\
b & 601 & 2027-06-17 & 6740.7118 & 0.0661 \\
c & 400 & 2027-06-20 & 6744.1717 & 0.2640 \\
b & 602 & 2027-06-25 & 6748.6343 & 0.0654 \\
c & 401 & 2027-07-02 & 6756.0675 & 0.2606 \\
b & 603 & 2027-07-03 & 6756.5548 & 0.0647 \\
b & 604 & 2027-07-10 & 6764.4758 & 0.0644 \\
c & 402 & 2027-07-14 & 6767.9643 & 0.2576 \\
b & 605 & 2027-07-18 & 6772.3982 & 0.0635 \\
c & 403 & 2027-07-26 & 6779.8617 & 0.2534 \\
b & 606 & 2027-07-26 & 6780.3186 & 0.0627 \\
b & 607 & 2027-08-03 & 6788.2393 & 0.0622 \\
c & 404 & 2027-08-07 & 6791.7604 & 0.2497 \\
b & 608 & 2027-08-11 & 6796.1613 & 0.0613 \\
c & 405 & 2027-08-19 & 6803.6596 & 0.2450 \\
b & 609 & 2027-08-19 & 6804.0812 & 0.0604 \\
b & 610 & 2027-08-27 & 6812.0015 & 0.0598 \\
c & 406 & 2027-08-31 & 6815.5604 & 0.2409 \\
b & 611 & 2027-09-04 & 6819.9233 & 0.0588 \\
c & 407 & 2027-09-11 & 6827.4615 & 0.2360 \\
b & 612 & 2027-09-12 & 6827.8431 & 0.0579 \\
b & 613 & 2027-09-20 & 6835.7630 & 0.0573 \\
c & 408 & 2027-09-23 & 6839.3645 & 0.2318 \\
b & 614 & 2027-09-28 & 6843.6844 & 0.0564 \\
c & 409 & 2027-10-05 & 6851.2676 & 0.2270 \\
b & 615 & 2027-10-06 & 6851.6037 & 0.0554 \\
b & 616 & 2027-10-14 & 6859.5231 & 0.0549 \\
c & 410 & 2027-10-17 & 6863.1728 & 0.2230 \\
b & 617 & 2027-10-21 & 6867.4443 & 0.0540 \\
c & 411 & 2027-10-29 & 6875.0779 & 0.2186 \\
b & 618 & 2027-10-29 & 6875.3634 & 0.0531 \\
b & 619 & 2027-11-06 & 6883.2826 & 0.0527 \\
c & 412 & 2027-11-10 & 6886.9852 & 0.2152 \\
b & 620 & 2027-11-14 & 6891.2034 & 0.0519 \\
c & 413 & 2027-11-22 & 6898.8923 & 0.2116 \\
b & 621 & 2027-11-22 & 6899.1220 & 0.0512 \\
b & 622 & 2027-11-30 & 6907.0407 & 0.0509 \\
c & 414 & 2027-12-04 & 6910.8016 & 0.2089 \\
b & 623 & 2027-12-08 & 6914.9611 & 0.0503 \\
c & 415 & 2027-12-16 & 6922.7106 & 0.2063 \\
b & 624 & 2027-12-16 & 6922.8797 & 0.0497 \\
b & 625 & 2027-12-24 & 6930.7981 & 0.0496 \\
c & 416 & 2027-12-28 & 6934.6217 & 0.2048 \\
b & 626 & 2028-01-01 & 6938.7184 & 0.0492 \\
c & 417 & 2028-01-09 & 6946.5325 & 0.2034 \\
b & 627 & 2028-01-09 & 6946.6365 & 0.0488 \\
b & 628 & 2028-01-17 & 6954.5545 & 0.0489 \\
c & 418 & 2028-01-20 & 6958.4451 & 0.2031 \\
b & 629 & 2028-01-24 & 6962.4744 & 0.0488 \\
c & 419 & 2028-02-01 & 6970.3573 & 0.2029 \\
b & 630 & 2028-02-01 & 6970.3924 & 0.0486 \\
b & 631 & 2028-02-09 & 6978.3103 & 0.0489 \\
c & 420 & 2028-02-13 & 6982.2712 & 0.2038 \\
b & 632 & 2028-02-17 & 6986.2302 & 0.0491 \\
b & 633 & 2028-02-25 & 6994.1479 & 0.0491 \\
c & 421 & 2028-02-25 & 6994.1847 & 0.2049 \\
b & 634 & 2028-03-04 & 7002.0654 & 0.0496 \\
c & 422 & 2028-03-08 & 7006.0996 & 0.2071 \\
b & 635 & 2028-03-12 & 7009.9850 & 0.0500 \\
b & 636 & 2028-03-20 & 7017.9027 & 0.0502 \\
c & 423 & 2028-03-20 & 7018.0140 & 0.2093 \\
b & 637 & 2028-03-28 & 7025.8202 & 0.0509 \\
c & 424 & 2028-04-01 & 7029.9296 & 0.2125 \\
b & 638 & 2028-04-05 & 7033.7397 & 0.0515 \\
b & 639 & 2028-04-13 & 7041.6574 & 0.0519 \\
c & 425 & 2028-04-13 & 7041.8446 & 0.2157 \\
b & 640 & 2028-04-21 & 7049.5747 & 0.0527 \\
c & 426 & 2028-04-25 & 7053.7605 & 0.2199 \\
b & 641 & 2028-04-28 & 7057.4940 & 0.0535 \\
b & 642 & 2028-05-06 & 7065.4116 & 0.0540 \\
c & 427 & 2028-05-07 & 7065.6759 & 0.2239 \\
b & 643 & 2028-05-14 & 7073.3289 & 0.0550 \\
c & 428 & 2028-05-19 & 7077.5918 & 0.2289 \\
b & 644 & 2028-05-22 & 7081.2484 & 0.0559 \\
b & 645 & 2028-05-30 & 7089.1661 & 0.0565 \\
c & 429 & 2028-05-31 & 7089.5071 & 0.2336 \\
b & 646 & 2028-06-07 & 7097.0834 & 0.0576 \\
c & 430 & 2028-06-11 & 7101.4228 & 0.2394 \\
b & 647 & 2028-06-15 & 7105.0027 & 0.0587 \\
b & 648 & 2028-06-23 & 7112.9204 & 0.0594 \\
c & 431 & 2028-06-23 & 7113.3376 & 0.2446 \\
b & 649 & 2028-07-01 & 7120.8378 & 0.0606 \\
c & 432 & 2028-07-05 & 7125.2528 & 0.2509 \\
b & 650 & 2028-07-09 & 7128.7573 & 0.0618 \\
b & 651 & 2028-07-17 & 7136.6754 & 0.0625 \\
c & 433 & 2028-07-17 & 7137.1668 & 0.2567 \\
b & 652 & 2028-07-25 & 7144.5929 & 0.0638 \\
c & 434 & 2028-07-29 & 7149.0812 & 0.2635 \\
b & 653 & 2028-08-02 & 7152.5123 & 0.0651 \\
b & 654 & 2028-08-09 & 7160.4305 & 0.0659 \\
c & 435 & 2028-08-10 & 7160.9942 & 0.2695 \\
b & 655 & 2028-08-17 & 7168.3481 & 0.0673 \\
c & 436 & 2028-08-22 & 7172.9076 & 0.2767 \\
b & 656 & 2028-08-25 & 7176.2678 & 0.0686 \\
b & 657 & 2028-09-02 & 7184.1864 & 0.0695 \\
c & 437 & 2028-09-03 & 7184.8192 & 0.2830 \\
b & 658 & 2028-09-10 & 7192.1042 & 0.0709 \\
c & 438 & 2028-09-15 & 7196.7313 & 0.2905 \\
b & 659 & 2028-09-18 & 7200.0239 & 0.0723 \\
b & 660 & 2028-09-26 & 7207.9427 & 0.0731 \\
c & 439 & 2028-09-27 & 7208.6414 & 0.2968 \\
b & 661 & 2028-10-04 & 7215.8607 & 0.0746 \\
c & 440 & 2028-10-09 & 7220.5521 & 0.3045 \\
b & 662 & 2028-10-12 & 7223.7808 & 0.0760 \\
b & 663 & 2028-10-20 & 7231.7001 & 0.0768 \\
c & 441 & 2028-10-20 & 7232.4603 & 0.3107 \\
b & 664 & 2028-10-28 & 7239.6184 & 0.0782 \\
c & 442 & 2028-11-01 & 7244.3696 & 0.3183 \\
b & 665 & 2028-11-05 & 7247.5386 & 0.0797 \\
b & 666 & 2028-11-12 & 7255.4581 & 0.0804 \\
c & 443 & 2028-11-13 & 7256.2757 & 0.3241 \\
b & 667 & 2028-11-20 & 7263.3766 & 0.0818 \\
c & 444 & 2028-11-25 & 7268.1833 & 0.3314 \\
b & 668 & 2028-11-28 & 7271.2970 & 0.0833 \\
b & 669 & 2028-12-06 & 7279.2172 & 0.0838 \\
c & 445 & 2028-12-07 & 7280.0874 & 0.3367 \\
b & 670 & 2028-12-14 & 7287.1361 & 0.0850 \\
c & 446 & 2028-12-19 & 7291.9932 & 0.3435 \\
b & 671 & 2028-12-22 & 7295.0567 & 0.0865 \\
b & 672 & 2028-12-30 & 7302.9771 & 0.0869 \\
c & 447 & 2028-12-31 & 7303.8951 & 0.3478 \\
b & 673 & 2029-01-07 & 7310.8962 & 0.0880 \\
c & 448 & 2029-01-12 & 7315.7991 & 0.3538 \\
b & 674 & 2029-01-15 & 7318.8171 & 0.0893 \\
b & 675 & 2029-01-23 & 7326.7381 & 0.0895 \\
c & 449 & 2029-01-24 & 7327.6987 & 0.3570 \\
b & 676 & 2029-01-31 & 7334.6577 & 0.0903 \\
c & 450 & 2029-02-05 & 7339.6010 & 0.3618 \\
b & 677 & 2029-02-08 & 7342.5789 & 0.0915 \\
b & 678 & 2029-02-16 & 7350.5001 & 0.0915 \\
c & 451 & 2029-02-16 & 7351.4984 & 0.3636 \\
b & 679 & 2029-02-23 & 7358.4198 & 0.0921 \\
c & 452 & 2029-02-28 & 7363.3988 & 0.3671 \\
b & 680 & 2029-03-03 & 7366.3412 & 0.0930 \\
b & 681 & 2029-03-11 & 7374.2630 & 0.0926 \\
c & 453 & 2029-03-12 & 7375.2942 & 0.3672 \\
b & 682 & 2029-03-19 & 7382.1831 & 0.0929 \\
c & 454 & 2029-03-24 & 7387.1930 & 0.3689 \\
b & 683 & 2029-03-27 & 7390.1049 & 0.0937 \\
b & 684 & 2029-04-04 & 7398.0269 & 0.0929 \\
c & 455 & 2029-04-05 & 7399.0863 & 0.3671 \\
b & 685 & 2029-04-12 & 7405.9471 & 0.0929 \\
c & 456 & 2029-04-17 & 7410.9836 & 0.3670 \\
b & 686 & 2029-04-20 & 7413.8690 & 0.0933 \\
b & 687 & 2029-04-28 & 7421.7914 & 0.0922 \\
c & 457 & 2029-04-29 & 7422.8753 & 0.3632 \\
b & 688 & 2029-05-06 & 7429.7121 & 0.0919 \\
c & 458 & 2029-05-11 & 7434.7713 & 0.3611 \\
b & 689 & 2029-05-14 & 7437.6342 & 0.0919 \\
b & 690 & 2029-05-22 & 7445.5569 & 0.0905 \\
c & 459 & 2029-05-23 & 7446.6615 & 0.3551 \\
b & 691 & 2029-05-29 & 7453.4775 & 0.0898 \\
c & 460 & 2029-06-04 & 7458.5564 & 0.3511 \\
b & 692 & 2029-06-06 & 7461.3997 & 0.0895 \\
b & 693 & 2029-06-14 & 7469.3226 & 0.0877 \\
c & 461 & 2029-06-15 & 7470.4456 & 0.3431 \\
b & 694 & 2029-06-22 & 7477.2435 & 0.0866 \\
c & 462 & 2029-06-27 & 7482.3398 & 0.3371 \\
b & 695 & 2029-06-30 & 7485.1659 & 0.0860 \\
b & 696 & 2029-07-08 & 7493.0890 & 0.0839 \\
c & 463 & 2029-07-09 & 7494.2282 & 0.3271 \\
b & 697 & 2029-07-16 & 7501.0098 & 0.0825 \\
c & 464 & 2029-07-21 & 7506.1222 & 0.3193 \\
b & 698 & 2029-07-24 & 7508.9321 & 0.0816 \\
b & 699 & 2029-08-01 & 7516.8552 & 0.0792 \\
c & 465 & 2029-08-02 & 7518.0102 & 0.3078 \\
b & 700 & 2029-08-09 & 7524.7761 & 0.0776 \\
c & 466 & 2029-08-14 & 7529.9043 & 0.2985 \\
b & 701 & 2029-08-17 & 7532.6986 & 0.0764 \\
b & 702 & 2029-08-25 & 7540.6217 & 0.0738 \\
c & 467 & 2029-08-26 & 7541.7924 & 0.2857 \\
b & 703 & 2029-09-02 & 7548.5425 & 0.0720 \\
c & 468 & 2029-09-07 & 7553.6869 & 0.2753 \\
b & 704 & 2029-09-09 & 7556.4646 & 0.0706 \\
b & 705 & 2029-09-17 & 7564.3876 & 0.0678 \\
c & 469 & 2029-09-19 & 7565.5755 & 0.2616 \\
b & 706 & 2029-09-25 & 7572.3083 & 0.0659 \\
c & 470 & 2029-09-30 & 7577.4708 & 0.2507 \\
b & 707 & 2029-10-03 & 7580.2305 & 0.0643 \\
b & 708 & 2029-10-11 & 7588.1536 & 0.0616 \\
c & 471 & 2029-10-12 & 7589.3602 & 0.2368 \\
b & 709 & 2029-10-19 & 7596.0740 & 0.0596 \\
c & 472 & 2029-10-24 & 7601.2567 & 0.2259 \\
b & 710 & 2029-10-27 & 7603.9958 & 0.0581 \\
b & 711 & 2029-11-04 & 7611.9185 & 0.0554 \\
c & 473 & 2029-11-05 & 7613.1471 & 0.2124 \\
b & 712 & 2029-11-12 & 7619.8387 & 0.0535 \\
c & 474 & 2029-11-17 & 7625.0451 & 0.2023 \\
b & 713 & 2029-11-20 & 7627.7605 & 0.0521 \\
b & 714 & 2029-11-28 & 7635.6831 & 0.0496 \\
c & 475 & 2029-11-29 & 7636.9369 & 0.1900 \\
b & 715 & 2029-12-06 & 7643.6031 & 0.0480 \\
c & 476 & 2029-12-11 & 7648.8365 & 0.1814 \\
b & 716 & 2029-12-14 & 7651.5243 & 0.0468 \\
b & 717 & 2029-12-21 & 7659.4466 & 0.0446 \\
c & 477 & 2029-12-23 & 7660.7298 & 0.1710 \\
b & 718 & 2029-12-29 & 7667.3662 & 0.0434 \\
